Nanodiamond grain boundaries and lattice expansion drive Silicon vacancy emission heterogeneity

Silicon-vacancy (SiV$^-$) centers in diamond are promising candidates as sources of single-photons in quantum networks due to their minimal phonon coupling and narrow optical linewidths. Correlating SiV$^-$ emission with the defect's atomic-scale structure is important for controlling and optimizing quantum emission, but remains an outstanding challenge. Here, we use cathodoluminescence imaging in a scanning transmission electron microscope (STEM) to elucidate the structural sources of non-ideality in the SiV$^-$ emission from nanodiamonds with sub-nanometer-scale resolution. We show that different crystalline domains of a nanodiamond exhibit distinct zero-phonon line (ZPL) energies and differences in brightness, while near-surface SiV$^-$ emitters remain bright. We correlate these changes with local lattice expansion using 4D STEM and diffraction, and show that associated blue shifts from the ZPL are due to defect density heterogeneity, while red shifts are due to lattice distortions.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}


# Uncomment this line to compile the differences in the SI
# $pdflatex = "latexdiff SI_Old.tex SI_Rev.tex > main-d.tex; pdflatex %O  main-d"


# Uncomment this line to compile the differences in the main text
# $pdflatex = "latexdiff Main_Old.tex Main_Rev.tex > main-d.tex; pdflatex %O  main-d"

==> output.tex <==



==> xx.tex <==


